Unsupervised Anomaly Detection with Adversarial Mirrored AutoEncoders

Detecting out of distribution (OOD) samples is of paramount importance in all Machine Learning applications. Deep generative modeling has emerged as a dominant paradigm to model complex data distributions without labels. However, prior work has shown that generative models tend to assign higher likelihoods to OOD samples compared to the data distribution on which they were trained. First, we propose Adversarial Mirrored Autoencoder (AMA), a variant of Adversarial Autoencoder, which uses a mirrored Wasserstein loss in the discriminator to enforce better semantic-level reconstruction. We also propose a latent space regularization to learn a compact manifold for in-distribution samples. The use of AMA produces better feature representations that improve anomaly detection performance. Second, we put forward an alternative measure of anomaly score to replace the reconstruction-based metric which has been traditionally used in generative model-based anomaly detection methods. Our method outperforms the current state-of-the-art methods for anomaly detection on several OOD detection benchmarks.

==> 2_background.tex <==
\section{Background}
\label{sec:Background}
\textcolor{red}{Is this section needed?}
This work considers the OOD detection in datasets with no class labels scenario.It is somewhat similar to One class classification/ One class Openset detection problems. Since anomalies are very rare in general, following the same setup as \cite{ruff2018deep, zenati2018adversarially, ren2019likelihood}, we assume that all data in the training set are normal samples. In appendix, we address the scenario in which the training data is corrupted with anomalies. \textcolor{red}{Maybe move it to main text, show the experiments with 5 percent anomalies}

Suppose we have an in-distribution dataset $\mathcal{D}_{in}$ consisting of $\{\bx_1, \bx_2,...\bx_m \}$ sampled from the distribution $\PP_{in}$. Our objective is to train our model $\mathcal{M}$ such that the anomaly score 




% Let $\mathbb{Q}_{X}$ be the distribution generating the anomaly samples. 
% In this paper, we consider the problem of identifying anomalies in a given dataset irrespective of their sources. Conventionally, anomalies are presumed to be generated by a different data distribution compared to that of the normal samples. For example, when we are dealing with CIFAR-10 images and an SVHN image is found in the mix, this would be an OOD anomaly. While in this example, there is a clear semantic shift, sometimes anomalies could just be inliers, i.e. they originate from the same manifold of the normal samples. For instance, when one class of CIFAR-10 is normal, rest 9 classes can be viewed as anomalous. For the sake of brevity, we use the same mathematical notation to refer to both in-distribution or out-of-distribution anomalies.



% \textcolor{red}{Remove this perhaps}
% \subsubsection{Abbreviations}

% Going forward, by normal samples we mean samples which are non-anomalous, or desired samples. We are \textit{not} referring to the Gaussian normal distribution. Also, we might use a shorthand AD for Anomaly detection, OOD for out-of-distribution, ID for in-distribution. 

